CRAB: Assessing the Strength of Causal Relationships Between Real-world Events

Understanding narratives requires reasoning about the cause-and-effect relationships between events mentioned in the text. While existing foundation models yield impressive results in many NLP tasks requiring reasoning, it is unclear whether they understand the complexity of the underlying network of causal relationships of events in narratives. In this work, we present CRAB, a new Causal Reasoning Assessment Benchmark designed to evaluate causal understanding of events in real-world narratives. CRAB contains fine-grained, contextual causality annotations for ~2.7K pairs of real-world events that describe various newsworthy event timelines (e.g., the acquisition of Twitter by Elon Musk). Using CRAB, we measure the performance of several large language models, demonstrating that most systems achieve poor performance on the task. Motivated by classical causal principles, we also analyze the causal structures of groups of events in CRAB, and find that models perform worse on causal reasoning when events are derived from complex causal structures compared to simple linear causal chains. We make our dataset and code available to the research community.

==> 03_method_long.tex <==
\section{Dataset Construction}

\label{par:data_collection}
In this section, we give an overview of causal event linking and its associated challenges and describe our approach for building \ourdata{} benchmark centered around these challenges.

\subsection{Overview}
\textbf{Notation:}
We are given a narrative $P$ (\eg, a part of a published news piece) covering a (part of a) news story $S$, that happened in a specific period of time.
Each narrative $P$ reports several events $\{E_{P1}, E_{P2}, \cdots, E_{PN}\}$
%$\{E_1, E_2,..., E_N\}_P$ 
associated with that story. 
% Note that a narrative's events are not ordered in any specific way.
With each story defining an order of its events (also called the story's ``timeline''), we build time-ordered lists of events extracted from the documents related to news stories: $[E_{S1}, E_{S2}, \cdots, E_{ST}]$. $T$ is the maximum order (\ie, the maximum time step) of the story's events.
%Note that events are not ordered in any specific way.
%Each story has a timeline $T$, which contains all the events extracted from the documents ordered in time $[E_{N_{i}1}, E_{N_{i}2}, ..., E_{N_{i}T}]$.

\noindent Besides, we define a (directed) causal graph of events, $G$, where nodes are individual events and a directed edge connects a head event and a tail event if and only if the head caused the tail. If a subset of $G$'s events
is extracted from the same document, we qualify their causal relations as in-document but cross-document causal paths can also be found in $G$.
%An event causal graph $G$ is made up of a set of interconnected events describing a story, each represented as a triple containing a head entity, a tail entity, and a causal relation connecting them. 
%The connected events can be related to the same (in-document) $(E_{iP_1}, E_{jP_1})$ or a different (cross-document) narrative $(E_{iP_1}, E_{jP_2})$.
Our goal is to identify the causal relations between events from $G$ based on the context (\ie, news pieces) these events refer to.

%\noindent \textbf{Challenges:}
Real-world causality identification and assessment poses several challenges:
%The task of real-world event causality identification and assessment poses several challenges:
%\begin{itemize}

%\item \textit{\textbf{Subjectivity: }}
\textbf{Subjectivity:} Assessing the actual causality of real-world events poses a great challenge in collecting causal judgments that are grounded in the narrative and not in the implicit knowledge and bias of the reader. 
People may feel a strong impression of causation about an event, even when the real causal relation is unclear based on the narrative \cite{wolff2013causation}.
Additionally, people with different backgrounds might disagree on the strength of the causal link between events, especially when these events are distant in time \cite{}. 


%\item \textit{\textbf{Contextualization: }}
\textbf{Contextualization:} Limited or subjective coverage of stories by the narratives makes the automated creation of the story timelines and the respective causal graphs subject to incompleteness.
For example, in Figure 1, if we didn't encounter the document with event \texttt{E2}, this event wouldn't be present in the timeline, and therefore, the causal reasoning step of \texttt{E1} to \texttt{E3} wouldn't be representative of the real-world situation.

%\item \textit{\textbf{Temporality: }}
\textbf{Temporality:} Extracting events from single narratives and ordering them based on their occurrence in time is a relatively straightforward task since we are grounding the extracted events on the timeline of a single document.
However, in the multi-document settings where the extracted events are grounded to different narratives published at different dates and whose respective timelines can be interleaved, the task of event linking and ordering becomes complex. 

%\end{itemize}

While many methods have been proposed for causal link identification and assessment, they mostly focus on binary commonsense causality detection across short spans of text (extracted from a single document), which does not adequately address the unique challenges of real-world causality judgment.
In the following sections, we present our approach for building \ourdata{} dataset that addresses the above challenges. 

\subsection{Narrative Selection}
We create a list of news stories about major events that happened around the globe during the past 10 years. This list is comprised of stories related to a variety of categories with events of geopolitical, social, and environmental nature.  
We created this list of stories both by crowdsourcing and by fact-checking various news sources manually. 
Based on a selection of 20 distinctive stories, and similarly to \cite{}, we crawl the web and select the top 20 news articles per story.

When extracting articles related to a story that happened years back in time, we noticed that the fetched articles covered also recent events that were loosely related to the main events of the story.
To eliminate these events, we use a time window of 9 months when extracting the articles for each story.
This serves as a filtering method in order to only extract articles that have been published around the time that the respective story happened.
Detailed descriptive statistics on stories and their categories as well as extensive information regarding the article extraction process, can be found in Appendix \ref{sec:appendix_art_selection} and in Table \ref{table:stories}.

To create the narratives $P$, we filter the extracted news articles and select the ones that have at least 100 tokens. 
We additionally filter out articles that have paywalls or provide re-directions to the original referred news article. 
Finally, we clip the article to 250 tokens and round to the end of the sentence token.
We end up using a total number of 384 news pieces as the main test bed for event extraction.

\subsection{Event Extraction} \label{event_exctraction}

For each of the selected news pieces, the goal is to identify the main events mentioned and create a set of the extracted events $\{E_{P1}, E_{P2}, \cdots, E_{PN}\}$ per narrative $P$. 
Compared to former extractive implementations of event identification from \cite{} and \cite{} that used Semantic Role Labeling (SRL) techniques to extract the event triggers and the associated arguments, we use a generative approach that outputs the main events given a news piece. 
We do so by prompting the GPT-$3.5$ (\ie, \texttt{text-davinci-003}) model \cite{brown2020language} with the article as context and additional instructions for information extraction generation similar to \cite{}.
An example of the event extraction prompt and the output is presented in \ref{sec:appendix_event_extraction}.

After extensive experimental analysis, we saw a twofold benefit of using a generative approach for event extraction.
First, when prompted correctly, generative models show satisfying performances in outputting structured information at the requested semantic abstraction. 
That led to higher precision results when extracting events and comparing them with the gold label of a sample of narratives that we had annotated.
Second, the semantic granularity of the events we wanted to extract is between sentence and document level, meaning that we aimed for the main events covered in the article and not syntactic events as existing works use. 
%For the Twitter acquisition example in Figure \ref{fig:example}, a semantic event in the desired granularity for our work is \textit{"Elon Musk sends a letter to Twitter proposing to move forward with the acquisition"} whereas a syntactic one derived from SLR tools is \textit{"Elon Musk proposes to move forward with the acquisition"}.

However, generative methods come with the limitation of hallucinations or invalid output.
We categorize the invalid events into error categories and perform both automated and manual filtering (see \ref{event_verification}) on the generated events in order to keep only the ones that clearly state an event that is referred to or implied by the news piece.
Table \ref{} showcases examples of failed event generations along with their error categories.

Overall, we confirm the findings of \cite{} and conclude that prompting LLMs for information extraction can leverage the trade-off between the syntactic consistency that extractive approaches guarantee and the semantic abstraction that generation provides. 
Additional implementation details and experiments regarding the different methods of event extraction that we tested can be found in \ref{sec:appendix_event_extraction}.

\subsection{Event Verification} \label{event_verification}
As mentioned in Section~\ref{event_exctraction}, when employing event extraction with GPT-3 in the loop, the extracted events might suffer from semantic or syntactic inconsistencies that lead to different error categories presented in Table \ref{}. 
To mitigate this and increase the quality of the extracted events respective to the context, we decided to use both automated and manual filtering approaches.
We first automatically filtered events that contain less than 3 tokens as this heuristic eliminates invalid and incoherent events. 
We also automatically removed generated events that represent claims or beliefs by filtering the utterances with conversational verbs followed by quotes (\eg, \textcolor{red}{TODO}).
For the manual filtering, two experts from our research group manually evaluated the validity of all the remaining generated events. 
The experts assessed the validity of the event based on the following categories: valid event, incoherent or unclear or wrong event, claim or belief or statement, and future event.
Further explanation and examples of these categories can be found in \ref{sec:appendix_event_ver}.

\begin{figure*}
    \includegraphics[width=\linewidth]{emnlp2023-latex/figures/dataset_overview.png}
    \caption{\label{fig:dataset}\ourdata{} data overview}
\end{figure*}

% After the event validity assessment, we additionally filtered out news pieces with no remaining events linked to them.
% We ended up keeping the X\% (X events) of original events and the X\% (X news pieces) of original news pieces.

\subsection{Timeline Construction}
It is essential to assess the causality of events whose occurrences in time are clearly ordered.   
% Since causality is conditioned over temporality, we wanted to assure the correct temporal order of events before assessing their pairwise causality. 
For each story, we created a timeline of the extracted events.
We prompted the gpt-davinci-003 LLM with an extracted event and the narrative reporting it, as well as an instruction asking for the event's date of occurrence.
% We prompt gpt-davinci-003 model giving as input the narratives of the story and the extracted events and requesting the date this event happened relative to the context. 
As an additional checking step, we manually curated the created timelines in order to assure their factual and temporal validity.

Note that events extracted from different narratives might actually be the same but expressed in a slightly different way. We observed that in particular, the main narrative's events are subject to this kind of duplication due to their multiple mentions in the news coverage.
%This is usually due to the fact that especially for main events, which are at the center of the story, the news coverage repeatedly mentions them and therefore we might have multiple narratives referring to the same instance of an event.
In order to tackle event disambiguation, we 
%perform event linking upon 
merged differently phrased instances of the same events during the creation of the timeline.
%keeping one instance of the event in the output timeline.
Post-annotation, we refer to the merged instances as one single node in the story graph $G$ while keeping all the textual versions pointing to this node available in the dataset, for the sake of completeness.

\subsection{Event Causality Linking}
The main challenge tackled here goes beyond in-document event detection and causality linking. 
We aim to link real-world events across different narratives and assess whether language models can perform cross-document causal reasoning among event pairs with different degrees of causality. 
To achieve this, we assess the links between all event pairs $\left(E_i, E_j\right)$ extracted from all the narratives $P$ related to a specific story $S$. % that are present in the timeline $T_s$. 
Note that since the events are extracted from various narratives, there will be pairs with events from the same narrative (in-document) and pairs with events originating from different narratives (cross-document) referring to the same story. 


% To assess the event pairs,
We then pass them to crowdworkers from Amazon Mechanical Turk in order to specify the events' causal relationships based on the given narrative according to the causal score described in Section \ref{par:preliminary}.
We run two experimental setups; one for in-document event pairs and one for cross-document event pairs.
\angie{[To be moved to Appendix:]For the in-document ones, we give the narrative along with 3 pairs.
For the cross-document ones, we give 2 narratives at a time along with 5 event pairs.
Figure \ref{fig:pipeline} depicts the pair creation process that served as input for Amazon Mechanical Turk experiments.}
Each pair in both setups is evaluated by 10 workers. 
More details regarding the qualification selection of the workers as well as the scripts provided for the experiment can be found in \ref{sec:appendix_crowdsourcing}.


